Security Wrappers for Information-Flow Control in Active Object Languages with Futures

This paper introduces a run-time mechanism for preventing leakage of secure information in distributed systems. We consider a general concurrency language model, where concurrent objects interact by asynchronous method calls and futures. The aim is to prevent leakage of confidential information to low-level viewers. The approach is based on the notion of a security wrapper, which encloses an object or a component and controls its interactions with the environment. A wrapper is a mechanism added by the run-time system to provide protection of an insecure component according to some security policies. The security policies of a wrapper are formalized based on a notion of security levels. At run-time, future components will be wrapped upon need, while only objects of unsafe classes will be wrapped, using static checking to limit the number of unsafe classes and thereby reducing run-time overhead. We define an operational semantics and prove that non-interference is satisfied. A service provider may use wrappers to protect its services in an insecure environment, and vice-versa: a system platform may use wrappers to protect itself from insecure service providers.

==> abs.tex <==
% \def\myttsize{\fontsize{8}{8}}   
\lstset{inputencoding=latin1,extendedchars,mathescape}
\lstset{basicstyle=\myttsize\sffamily}
\lstset{numberstyle=\small%\tiny
}%
\lstset{language=}
\lstset{emphstyle=\color{red},emphstyle={[2]\color{blue}\underbar}}%% global
\lstset{
numbers=left, 
numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\small%\tiny%\color{mygray}
} 


%% ABS
\lstdefinelanguage{ABS}{keywords=
{Any,var,op,Nil,null,this,thisDC,yield,dyndelta,new,data,type,def,case,of,cog,class,interface,extends,implements,if,else,await,get,total,load,transfer,movecogto,Fut,return,skip,while,module,duration,now,deadline,import, export, uses, from,local, suspend,delta,adds,modifies,removes,original,productline,features,core,corefeatures,optionalfeatures,after,when,product,hasAttribute,hasMethod,root,extension,group,allof,oneof,require,exclude,original,ifin,ifout,opt,spawn,newgroup,acquire,in,except,joins,leaves,as,subtypeOf}, sensitive=true, comment=[l]{//}, morecomment=[s]{/*}{*/}, morestring=[b]"}

%\def\codesize{\fontsize{9}{10}}

\lstdefinestyle{absstyle}{
language=ABS,columns=fullflexible,
 		   mathescape=true,%
 		   showstringspaces=false,%
keywordstyle=\bf\sffamily,
commentstyle=\sl\sffamily,%
basicstyle=\footnotesize\sffamily,
inputencoding=latin1, % i would prefer utf8
extendedchars,xleftmargin=2em
}

% \lstnewenvironment{abs}[1][]{%
%  \lstset{style=absstyle,#1}%
%    \csname lst@SetFirstLabel\endcsname}
%   {\csname lst@SaveFirstLabel\endcsname}

% \newcommand{\Abs}[1]{%
%   \lstinline[language=ABS,mathescape=true,%
%            keywordstyle=\bf\sffamily,%
%            basicstyle=\normalsize\sffamily,inputencoding=latin1, % i would prefer utf8
%            extendedchars]!#1!}
%   {\csname lst@SaveFirstLabel\endcsname}

\newcommand{\Abs}[1]{\lstinline[language=ABS,columns=fullflexible,mathescape=true,inputencoding=latin1,extendedchars,keywordstyle=\bf\sffamily,basicstyle=\myabsinlinesize\sffamily]!#1!}

\newcommand{\Absmath}[1]{\mbox{\lstinline[language=ABS,columns=fullflexible,mathescape=true,inputencoding=latin1,extendedchars,keywordstyle=\bf\sffamily,basicstyle=\myabsmathsize\sffamily]!#1!}}

\newenvironment{absinline}[1][]{%
\lstset{language=ABS,
		 showstringspaces=false,
		 columns=fullflexible,mathescape=true,%
         keywordstyle=\bf\sffamily,commentstyle=\sl\sffamily,%
         basicstyle=\normalsize\sffamily,inputencoding=latin1, % i would prefer utf8
         extendedchars,xleftmargin=2em,#1}}
{}

\newcommand{\absshow}[1]{%
\absinline{\lstinputlisting{code/#1}}
}

\newenvironment{abscolumn}{\\\mbox{}\hspace{12pt}\rule{0.95\linewidth}{0.5pt}%\noindent\mbox{}\noindent\hrulefill
\\}{\\\mbox{}\hspace{12pt}\rule{0.95\linewidth}{0.5pt}
% \\\noindent\mbox{}\hrulefill\mbox{}
}

\lstnewenvironment{absexample}{
~\\
\noindent 
\small{\textcolor{Green!80!black}{\bfseries\sffamily{Example:}}}\vspace{-4pt}
\lstset{style=absstyle,
basicstyle=\myttsize\sffamily,
framerule=1pt,
backgroundcolor=\color{Green!5},
rulecolor=\color{Green!80!black},
frame=tblr,
xleftmargin=4pt,
}}
{}

\lstnewenvironment{absexamplen}[1][]{
\lstset{style=absstyle,
basicstyle=\myttsize\sffamily,
framerule=1pt,tabsize=2,
backgroundcolor=\color{Green!5},
rulecolor=\color{Green!80!black},
frame=tblr,
captionpos=b,
xleftmargin=4pt,#1
}}
{}

